An Exploratory Survey of Hybrid Testing Techniques Involving Symbolic Execution and Fuzzing

Recent efforts in practical symbolic execution have successfully mitigated the path-explosion problem to some extent with search-based heuristics and compositional approaches. Similarly, due to an increase in the performance of cheap multi-core commodity computers, fuzzing as a viable method of random mutation-based testing has also seen promise. However, the possibility of combining symbolic execution and fuzzing, thereby providing an opportunity to mitigate drawbacks in each other, has not been sufficiently explored. Fuzzing could, for example, expedite path-exploration in symbolic execution, and symbolic execution could make seed input generation in fuzzing more efficient. There have only been, in our view, very few hybrid solution proposals with symbolic execution and fuzzing at their centre. By analyzing 77 relevant and systematically selected papers, we (1) present an overview of hybrid solution proposals of symbolic execution and fuzzing, (2) perform a gap analysis in research of hybrid techniques to improve both, plain symbolic execution and fuzzing, (3) propose new ideas for hybrid test-case generation techniques.

==> sections/introduction-old.tex <==
\vspace{-1ex}\section{Introduction}\label{sec:introduction}
Blackbox fuzzing \cite{sutton2007fuzzing} and symbolic execution \cite{king1976symbolic} are well-known methods of software testing, which have been intensively researched over the past couple of decades as techniques for finding bugs in software and generating test cases. Blackbox fuzzing (or, simply, \emph{fuzzing}) is, broadly speaking, an automated technique of random testing infused with monitoring mechanisms to decide \emph{mutations} for initial \emph{seed inputs}, so as to uncover previously unseen functionality. Symbolic execution is a technique to deterministically analyze the program under test by enumerating the paths as constraint systems, that are solved (using constraint solvers) to generate test cases that execute corresponding paths. Whitebox fuzzing \cite{godefroid2008automated} is a practical approach to symbolic execution that uses seed inputs, like blackbox fuzzing, to record some initial constraints of a program which are sequentially negated to form new constraints and solved to generate new test cases. While, due to its automation, fuzzing is a fast way to find many easy bugs it has been shown \cite{sutton2007fuzzing} to be ineffective in finding bugs in complex program constructs. On the other hand, even though symbolic execution is effective in covering unique (even complex) paths, its efficiency suffers from the bottlenecks of constraint solvers, such as SMT. 

Due to similarity in their goals, fuzzing and symbolic execution (or whitebox fuzzing) have the potential to be used as mutually beneficial methods of discovering vulnerabilities, as effectively demonstrated in \cite{pak2012hybrid}. In this paper, we aim to get an overview of the field of \emph{vulnerability detection techniques that incorporate both, fuzzing and symbolic execution}. The rest of the paper is divided as follows -- \Cref{sec:method} gives an overview of our research questions and the methodology of collecting and analyzing literature in this field. In \cref{sec:results} we try to answer all our research questions, and discuss in detail our key insights about research in this area. \Cref{sec:background} gives some background into the general fields of fuzzing and symbolic execution, and in \cref{sec:conclusion} we conclude our paper. 
